Efficient Backdoor Removal Through Natural Gradient Fine-tuning

The success of a deep neural network (DNN) heavily relies on the details of the training scheme; e.g., training data, architectures, hyper-parameters, etc. Recent backdoor attacks suggest that an adversary can take advantage of such training details and compromise the integrity of a DNN. Our studies show that a backdoor model is usually optimized to a bad local minima, i.e. sharper minima as compared to a benign model. Intuitively, a backdoor model can be purified by reoptimizing the model to a smoother minima through fine-tuning with a few clean validation data. However, fine-tuning all DNN parameters often requires huge computational costs and often results in sub-par clean test performance. To address this concern, we propose a novel backdoor purification technique, Natural Gradient Fine-tuning (NGF), which focuses on removing the backdoor by fine-tuning only one layer. Specifically, NGF utilizes a loss surface geometry-aware optimizer that can successfully overcome the challenge of reaching a smooth minima under a one-layer optimization scenario. To enhance the generalization performance of our proposed method, we introduce a clean data distribution-aware regularizer based on the knowledge of loss surface curvature matrix, i.e., Fisher Information Matrix. Extensive experiments show that the proposed method achieves state-of-the-art performance on a wide range of backdoor defense benchmarks: four different datasets- CIFAR10, GTSRB, Tiny-ImageNet, and ImageNet; 13 recent backdoor attacks, e.g. Blend, Dynamic, WaNet, ISSBA, etc.

==> eval_fisher.tex <==
% \begin{table}[!htp]
% \renewcommand{\arraystretch}{1.1}
% \renewcommand\tabcolsep{1.75pt}
% \small
% \centering
% \caption{The attack success rate (ASR) and the clean accuracy (CA)  of 4 backdoor defense methods against 10 backdoor attacks including 3 label poisoning attacks, 2 clean label attacks and 2 optimization attacks. \emph{None} means the training data is completely clean.}
%   \label{tab1}
% \scalebox{1}{
% \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{\begin{tabular}[c|]{@{}c@{}}No Defense\end{tabular}} & \multicolumn{2}{c|}{FP} & \multicolumn{2}{c|}{MCR} & \multicolumn{2}{c|}{NAD} & \multicolumn{2}{c|}{ANP} &  \multicolumn{2}{|c}{\textbf{NGF (Ours)}}\\ \cline{3-14} 
%  &  & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC \\ \hline
% \multirow{8}{*}{\footnotesize CIFAR-10} 
% & \emph{None} & 0 & 95.26 & 0 & 88.92  & 0 & 90.32 & 0 & 92.71 & 0 & 94.53  & 0 & 95.14  \\ %\cline{2-12}
% & BadNets &  100 & 90.93 & 98.12 & 85.62 & 3.99 & 81.85 & 4.39 & 85.61 & 2.94 & 84.88  & 1.69 & 85.79 \\
% & Blend & 100 & 93.98  & 62.57 & 84.37 & 32.77 & 80.39 & 5.28 & 84.99 & 3.84 & 89.20  & 0.36 & 90.23 \\
% % & Trojan-one & 100 & 88.63  & 82.86 & 83.31 & 20.55 & 79.83  & 17.61 &  83.66 & 5.73 & 84.94  & 2.93 & 87.20 \\
% & Trojan & 100 & 90.67 & 80.31 & 84.93 & 22.84 & 80.88  & 18.71 & 83.57 & 5.44 & 85.34 & 2.68 & 84.81 \\
% & SIG & 99.75 & 88.64 & 69.92 & 84.51 & 0.91  & 82.44  & 2.17 & 84.77 & 0.39 & 84.63 &  0.31 & 83.14 \\
%  & Dynamic & 100 & 92.52  & 79.14 & 84.07 & 24.83 & 78.69 & 23.29 & 82.61 & 5.75 & 85.36 & 8.90 & 91.16 \\
% %  & Dynamic-all & 100 & 92.14 & 80.43 & 83.61 & 26.32 & 77.85 & 22.66 & 81.11 & 2.29 & 84.61  & 0.64& 90.35  \\
%  &   CLB & 98.72 & 89.18 & 46.17 & 84.15 & 34.74 & 79.56 & 16.11 & 84.12 & 1.48 & 84.02 & 1.04 & 83.10\\  %\\ \cline{2-12} 
%   & FC & 87.85 & 84.69 & 62.14 & 82.47  &  40.81 & 81.75 & 53.42 & 83.64 & 3.61 & 82.77 & 3.18 & 82.97 \\\cline{2-12} 
%  & \multicolumn{1}{l}{Average Drop} & \multicolumn{1}{|l}{97.83} & \multicolumn{1}{l}{83.55} & \multicolumn{1}{|l}{75.07} & \multicolumn{1}{l}{80.62} & \multicolumn{1}{|l}{24.38} & \multicolumn{1}{l}{76.56} & \multicolumn{1}{|l}{20.40} & \multicolumn{1}{l}{80.37}  & \multicolumn{1}{|c}{\textbf{7.69}} & \multicolumn{1}{c}{\textbf{84.76}} \\ \midrule
% \multirow{6}{*}{GTSRB} 
%   & \emph{None} & 0 & 97.87 & 0 & 90.14 & 0 & 95.49 &  0 & 95.18 &  0 & 96.12 & 0 & 96.70 \\
%   & Badnets & 100 & 97.38 & 99.57 & 88.61 &  1.00 & 93.45 & 0.19 & 89.52 & 0.43 & 93.31 &  0.04 & 94.25 \\
%   & Blend & 100 & 95.92 & 99.50 & 86.67 & 6.83 & 92.91 & 8.10 & 89.37 & 4.09 & 93.14 & 0.11 & 93.39  \\
% %   & Troj-one & 99.50 & 96.27 &  93.54 & 84.22 & 2.76 & 92.98 & 0.37 & 90.02 & 0.81 & 92.74 & 0.36 & 94.95 & 0.21 &  95.18  \\
%   &  Trojan & 99.71 & 96.08 & 94.82 & 84.03 & 3.25 & 92.18  & 0.98 & 90.27 & 1.11 & 92.63 & 0.69 & 93.87 \\
%   &  SIG & 97.13 & 96.93 & 79.28 & 90.50 & 33.98 & 91.83 & 4.64 & 89.36 & 5.21 & 91.82 & 1.08 & 93.15  \\
%   &  Dynamic & 100 & 97.27 & 99.84 & 88.38 & 64.82 & 43.91 & 68.71 & 76.93 & 2.23 & 93.15 & 1.65 & 95.09 \\
% %   &  Dyn-all & 100 & 97.05 & 99.50 & 88.51 & 66.31 & 45.46 & 67.73 & 77.42 & 2.49 & 92.89 & 7.03 & 95.62 & 0.26 & 95.94 \\
% %  & CLB & 99.83\% & 83.43\% & 54.95\% & 81.53\% & 19.86\% & 77.36\% & 16.11\% & 80.73\% & \textbf{0\%} & \textbf{89.03\%} \\ 
% %   & FC & 88.52\% & 83.3& \textbf{29.81\%} & \textbf{84.66\%}
%   \cline{2-12}  
%   & \multicolumn{1}{l}{Average Drop} & \multicolumn{1}{|l}{97.73} & \multicolumn{1}{l}{83.55} & \multicolumn{1}{|l}{75.07} & \multicolumn{1}{l}{80.62} & \multicolumn{1}{|l}{24.38} & \multicolumn{1}{l}{76.56} & \multicolumn{1}{|l}{20.40} & \multicolumn{1}{l}{80.37}  & \multicolumn{1}{|c}{\textbf{7.69}} & \multicolumn{1}{c}{\textbf{84.76}} \\ 

%  \bottomrule
% \end{tabular}}
% \vspace{-0.1in}
% \end{table}

% \begin{table}[ht]
%     \centering
%     \caption{Performance comparison of NGF on ImageNet Dataset.}
%     \scalebox{0.95}{
%     \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
%     \toprule
% {\begin{tabular}[c|]{@{}c@{}}No Defense\end{tabular}} & \multicolumn{2}{c|}{FP} & \multicolumn{2}{c|}{MCR} & \multicolumn{2}{c|}{NAD} & \multicolumn{2}{c|}{ANP} &  \multicolumn{2}{|c}{\textbf{NGF (Ours)}}\\ \cline{3-14} 
%   & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC \\ \hline \\
%     \midrule

%     None & 0 & 91.1 & & & &  & & & &  & &  \\
%     Badnets & & & &  & & & &  & & & & \\
%     Blend & & & &  & & & &  & & & & \\
%     Trojan & & & &  & & & &  & & & & \\
%     Dynamic & & & &  & & & &  & & & & \\
%     SIG & & & &  & & & &  & & & & \\
%     CLB & & & &  & & & &  & & & & \\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:different_optimizer}
% \end{table}





% \begin{table}[!tp]
% \renewcommand{\arraystretch}{1.1}
% \renewcommand\tabcolsep{1.75pt}
% \small
% \centering
% \caption{\footnotesize Performance of NGF on CIFAR10 dataset under 7 different backdoor attacks while fine-tuning the classification layer with only $1\%$ of clean validation data. NGF achieves SOTA performance for 6 attacks while sacrificing only $4.19\%$ in clean accuracy (ACC) on average. The average drop indicates the difference in values before and after removal. Higher ASR drop and lower ACC drop is desired for a good defense mechanism.}
%   \label{tab:cifar_defense}
% \scalebox{0.825}{
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% Attacks & 
% %  \multicolumn{2}{c|}{\begin{tabular}[c|]{@{}c@{}}None\end{tabular}} & \multicolumn{2}{c|}{BadNets} &
% \multicolumn{2}{c|}{None} & \multicolumn{2}{c|}{BadNets} &
% \multicolumn{2}{c|}{Blend} & \multicolumn{2}{c|}{Trojan} & \multicolumn{2}{c|}{SIG} &  \multicolumn{2}{c|}{Dynamic}&  \multicolumn{2}{c|}{CLB}&  \multicolumn{2}{c|}{FC}&\multicolumn{2}{c}{Avg. Drop}\\ 
% \midrule%\cline{3-20} 
% Defenses&ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC& ASR &ACC & ASR &ACC & ASR &ACC \\ \midrule
% % \multirow{8}{*}{\rotatebox[origin=c]{90} {CIFAR-10}} 
% % & 
% \emph{No Defense} & 0 & 95.26 & 100 & 90.93  & 100 & 93.98 & 100 & 90.67 & 99.75 & 88.64  & 100 & 92.52&98.72&89.18&87.85&84.69&-&-   \\ %\cline{2-12}
%  FT & 0 & 92.28 & 4.87 & 82.65 & 21.81 & 80.12 & 3.78 & 81.21 & 2.04 & 80.18 & 11.73 & 81.14 & 2.89 & 80.22 & 4.12 & 78.61 &90.72$\downarrow$ &9.49$\downarrow$ \\
%  FP &  0 & 88.92 & 98.12 & 85.62 & 62.57 & 84.37 & 80.31 & 84.93 & 69.92 & \textbf{84.51}  & 79.14&84.07&46.17&\textbf{84.15}&62.14&82.47&26.85$\downarrow$&5.77$\downarrow$ \\
%  MCR & 0&90.32&3.99&81.85&32.77&80.39&22.84&80.88&0.91&82.44&24.83&78.69&34.74&79.56&40.81&81.75&75.05$\downarrow$&9.29$\downarrow$ \\
% % & Trojan-one & 100 & 88.63  & 82.86 & 83.31 & 20.55 & 79.83  & 17.61 &  83.66 & 5.73 & 84.94  & 2.93 & 87.20 \\
%  NAD & 0&92.71&4.39&85,61&5.28&84.99&18.71&83.57&2.17&83.77&23.29&82.61&16.11&84.12&53.42&82.64&80.41 $\downarrow$ &5.89 $\downarrow$\\
%  ANP & 0&\textbf{93.53}&2.94&84.88&3.84&89.20&5.44&\textbf{85.34}&0.39&83.63&\textbf{5.75}&85.36&1.48&84.02&3.61&82.77&94.69 $\downarrow$ & 4.91 $\downarrow$ \\
%   NGF(Ours) & 0&92.97&\textbf{1.69}&\textbf{85.79}&\textbf{0.36}&\textbf{90.23}&\textbf{2.68}&84.81&\textbf{0.31}&84.14&8.90&\textbf{91.16}&\textbf{1.04}&83.10&\textbf{3.18}&\textbf{82.97}&\textbf{95.44} $\downarrow$ &\textbf{4.05} $\downarrow$ \\

%  \bottomrule
% \end{tabular}}
% \vspace{-0.1in}
% \end{table}


% \begin{table}[!tp]
% \renewcommand{\arraystretch}{1.1}
% \renewcommand\tabcolsep{1.75pt}
% \small
% \centering
% \caption{\footnotesize Performance comparison of NGF and 5 other defense methods for GTSRB dataset. The average drop in ASR and ACC determines the effectiveness of a defense method.}
% \label{tab:gtsrb_defense}
% \scalebox{0.825}{
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% Attacks & \multicolumn{2}{c|}{None} & \multicolumn{2}{c|}{BadNets} & \multicolumn{2}{c|}{Blend} & \multicolumn{2}{c|}{Trojan} & \multicolumn{2}{c|}{SIG} &  \multicolumn{2}{|c}{Dynamic}&\multicolumn{2}{|c}{Avg. Drop}\\ \midrule
% Defenses&ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC& ASR &ACC  \\ \midrule
% % \multirow{8}{*}{\rotatebox[origin=c]{90} {CIFAR-10}} 
% % & 
% \emph{No Defense} & 0&97.87&100&97.38&100&95.92&99.71&96.08&97.13&96.93&100&97.27&-&-  \\ %\cline{2-12}
%  FT & 0 & 93.08 & 1.36 & 86.16 & 5.08 & 87.32 & 2.07 & 89.45 & 1.93 & 90.41 & 6.27 & 90.26 & 96.25$\downarrow$& 7.99$\downarrow$  \\
%  FP &  0&90.14&99.57&88.61&99.50&86.67&94.82&84.03&79.28&90.50&99.84&88.38&4.76$\downarrow$&9.06$\downarrow$ \\
%  MCR & 0&95.49&1.00&93.45&6.83&92.91&3.25&92.18&33.98&91.83&64.82&43.91&77.38$\downarrow$&13.84$\downarrow$ \\
% % & Trojan-one & 100 & 88.63  & 82.86 & 83.31 & 20.55 & 79.83  & 17.61 &  83.66 & 5.73 & 84.94  & 2.93 & 87.20 \\
%  NAD & 0&95.18&0.19&89.52&8.10&89.37&0.98&90.27&4.64&89.36&68.71&76.93&82.83$\downarrow$&9.62$\downarrow$ \\
%  ANP & 0&95.12&0.43&93.31&4.09&93.14&1.11&92.63&5.21&91.82&2.23&93.15&96.75$\downarrow$&3.89$\downarrow$\\
%   NGF(Ours) & 0&\textbf{95.65}&\textbf{0.04}&\textbf{94.25}&\textbf{0.11}&\textbf{93.39}&\textbf{0.69}&\textbf{93.87}&\textbf{1.08}&\textbf{93.15}&\textbf{1.65}&\textbf{95.09}&\textbf{98.65} $\downarrow$&\textbf{2.76}$\downarrow$ \\

%  \bottomrule
% \end{tabular}}
% \vspace{-0.1in}
% \end{table}



% \begin{table}[!htp]
% \renewcommand{\arraystretch}{1.1}
% \renewcommand\tabcolsep{1.75pt}
% \small
% \centering
% \caption{Main ImageNet Subset}
%   \label{tab1:CIFAR10}
% \scalebox{1}{
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c|}{\begin{tabular}[c|]{@{}c@{}}None\end{tabular}} & \multicolumn{2}{c|}{BadNets} & \multicolumn{2}{c|}{Blend} & \multicolumn{2}{c|}{Trojan} & \multicolumn{2}{c|}{SIG} &  \multicolumn{2}{|c}{Dynamic}&  \multicolumn{2}{|c}{CLB}&  \multicolumn{2}{|c}{FC}&\multicolumn{2}{|c}{Avg. Drop}\\ %\cline{3-20} 
% &ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC & ASR &ACC& ASR &ACC & ASR &ACC & ASR &ACC \\ \hline
% % \multirow{8}{*}{\rotatebox[origin=c]{90} {CIFAR-10}} 
% % & 
% \emph{No Defense} & 0 & 95.26 & 0 & 88.92  & 0 & 90.32 & 0 & 92.71 & 0 & 94.53  & 0 & 95.14  \\ %\cline{2-12}
%  FP &  100 & 90.93 & 98.12 & 85.62 & 3.99 & 81.85 & 4.39 & 85.61 & 2.94 & 84.88  & 1.69 & 85.79 \\
%  MCR & 100 & 93.98  & 62.57 & 84.37 & 32.77 & 80.39 & 5.28 & 84.99 & 3.84 & 89.20  & 0.36 & 90.23 \\
% % & Trojan-one & 100 & 88.63  & 82.86 & 83.31 & 20.55 & 79.83  & 17.61 &  83.66 & 5.73 & 84.94  & 2.93 & 87.20 \\
%  NAD & 100 & 90.67 & 80.31 & 84.93 & 22.84 & 80.88  & 18.71 & 83.57 & 5.44 & 85.34 & 2.68 & 84.81 \\
%  ANP & 99.75 & 88.64 & 69.92 & 84.51 & 0.91  & 82.44  & 2.17 & 84.77 & 0.39 & 84.63 &  0.31 & 83.14 \\
%   NGF(Ours) & 100 & 92.52  & 79.14 & 84.07 & 24.83 & 78.69 & 23.29 & 82.61 & 5.75 & 85.36 & 8.90 & 91.16 \\

%  \bottomrule
% \end{tabular}}
% \vspace{-0.1in}
% \end{table}

==> experimental_results_augmentation.tex <==
\section{Experimental Results}


\begin{table}[ht]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
    \toprule
    Method & \multicolumn{2}{c|}{No Defense} & \multicolumn{2}{c|}{FP} & \multicolumn{2}{c|}{MCR} & \multicolumn{2}{c|}{NAD} & \multicolumn{2}{c|}{ABL} & \multicolumn{2}{c}{FIR} \\
    \midrule
    Attacks & ASR & ACC & ASR & ACC & ASR & ACC & ASR & ACC & ASR & ACC & ASR & ACC \\
    \midrule
    None & 0 & 91.1 & & & &  & & & &  & &  \\
    Badnets & & & &  & & & &  & & & & \\
    Blend & & & &  & & & &  & & & & \\
    Trojan-one & & & &  & & & &  & & & & \\
    Trojan-all & & & &  & & & &  & & & & \\
    SIG & & & &  & & & &  & & & & \\
    Dynamic-one & & & &  & & & &  & & & & \\
    Dynamic-all & & & &  & & & &  & & & & \\
    CLB & & & &  & & & &  & & & & \\
    Feature & & & &  & & & &  & & & & \\
    FC & & & &  & & & &  & & & & \\    

    \bottomrule
    \end{tabular}}
    \vspace{2mm}
    \caption{Comparison of different defense methods for poisoned CIFAR10 dataset. We use 10 diffetrent attacks with a wide range of attacking strategies to show the effectiveness of FIR.}
    \label{tab:cifar10_defense}
\end{table}


\begin{table}[ht]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
    \toprule
    Method & \multicolumn{2}{c|}{No Defense} & \multicolumn{2}{c|}{FP} & \multicolumn{2}{c|}{MCR} & \multicolumn{2}{c|}{NAD} & \multicolumn{2}{c|}{ABL} & \multicolumn{2}{c}{FIR} \\
    \midrule
    Attacks & ASR & ACC & ASR & ACC & ASR & ACC & ASR & ACC & ASR & ACC & ASR & ACC \\
    \midrule
    None & 0 & 91.1 & & & &  & & & &  & &  \\
    Badnets & & & &  & & & &  & & & & \\
    Blend & & & &  & & & &  & & & & \\
    Trojan-one & & & &  & & & &  & & & & \\
    Trojan-all & & & &  & & & &  & & & & \\
    SIG & & & &  & & & &  & & & & \\
    Dynamic-one & & & &  & & & &  & & & & \\
    Dynamic-all & & & &  & & & &  & & & & \\
    CLB & & & &  & & & &  & & & & \\
    Feature & & & &  & & & &  & & & & \\
    FC & & & &  & & & &  & & & & \\   
    \bottomrule
    \end{tabular}
    }
    \vspace{2mm}
    \caption{Comparison of different defense methods for poisoned GTSRB dataset. We use 10 different attacks with a wide range of attacking strategies to show the effectiveness of FIR.}
    \label{tab:gtsrb_defense}
\end{table}



==> queries.tex <==
\section{Questions \& Answers}

We need to address following questions related to our proposed method:
\begin{itemize}
    \item What is relation/differences between adversarial input perturbation method and strong input augmentation method?
    
    \item \textbf{Answer:} Already did the experiment. Explain the results. In contrast to perturbation, Training cost is zero for our method. Our strong augmentation covers all possible perturbations (show graphically and using tables). Theoritical justification!!
    
    \item What would happen if the backdoored model is trained with strong augmentation data set? Does still  the proposed method work? 
    
    \item \textbf{Answer:} Strong/stronger augmentation can cleanse strongly augmented backdoored model. Show experimental evaluation. Theoritical explanation can be found in the training scheme. If we do not change the labels while adding augmentations, it will regularize the model which is opposite of the backdooring(de-regularization/memorization). a) Changing labels while augmenting is similar as de-regularizing. b) Difference between weak and strong augmentation while backdooring can give us some hint about the nature of backdoor insertion!!!  
    
    \item What are the augmentation types that remove backdoor? Is their any relation between augmentation types and backdoored model type?
    
    \item \textbf{Answer:} We will use 10/15 different augmentations and show their impact on backdoor removal. Then we will create 20 different combinations of augmentations and see what happens.

    \item  Can we show the attribution of (triggered) input that results the label corresponding to backdoored and backdoored-removed model? Does it reflect the trigger-agnostic (or, generalization) learning after backdoor removal? 
    
    \item \textbf{Answer:} we can generate the decision heatmap for some trigger and clean images. That will give us the indication whther augmentation has removed the backdoor.  
    
    \item Can \textbf{adversarial neural pruning} collapse the network itself? Can strong augmentation-based training protect network collapse?
    
    \item \textbf{Answer:} We can take an example where neural pruning can lead to layer collapse. (This is optional)
    
    \item Relationship between size of the model and attack success rate? See Odyssey
    
    \item Triggering data is another type of augmentation.
    
    
\end{itemize}

\textbf{Trigger Distribution.} 

Q. How does the (augmentation-based) proposed approach remove backdoor corresponding to Gaussian noise based trigger??  








\section{Discussion on Existing papers.}

\textbf{Sharpness-Aware Minimization (SAM)~\cite{foret2021sharpnessaware}.} Typical optimization procedures (e.g., SGD, ADAM) can optimize (minimize loss of) the model to a local/global minima which can significantly differ than the minima corresponding to model generalization loss for the input data distribution (Note, training data set is a only a subset of the general input data distribution). SAM proposed to optimize both the loss function ($l(w)$) and changes of loss function from neighbour weights ($l(w+\epsilon) - l(w)$) so that the optimizer will aware of sharp changes in weight loss landscape.  

\textbf{Adversarial Weight Perturbation (AWP)~\cite{wu2020adversarial}.}



==> rebuttal.tex <==
-------------------------------------------------------------------------------

Three questions:
Why does only the last layer remove the backdoor?
Why does NGD perform better than other optimizers?
Big accuracy drops? 

Motivation:

Working Principles: 

========================================================================

R1

========================================================================


Q1: Any insights into why NGD works so well while other optimizers perform poorly?
Q2: Could you also include results for larger models and larger datasets?
Q3: In Table 6, why is NGF only 2x faster than vanilla FT while it only needs to fine-tune one layer?
Can we show the computational burden of NGD and SGD for the same number of parameters? With references. With equations too.
-----------------------------------------------------------------------------------------------------
***

**Response for Q1:**

*Insights into why NGD works so well:* NGD is a loss surface geometry-aware optimizer that helps it to skip local minima. In case of one layer fine-tuning, the optimization problem intuitively becomes an under-parameterized model containing ***bad local minima***. In such a case, SGD and its variants most probable get stuck in those bad local minima performing poorly for the optimization problem [18,19]. In contrast, due to the geometry awareness of NGD, it can easily avoid local minima. Therefore, NGD performs so well than the first-order optimizers. 

From another point of view, NGD helps to generate a flat weight landscape surface which makes the fine-tuned DNN model more robust against the poisoned samples. We hypothesize that the loss surface geometry awareness of NGD helps it to flatten the landscape. The experimental loss landscapes corresponding to our hypothesis are presented in Fig. 1 which support our claim.

***
***
**Response for Q2:**

We have evaluated our method on ImageNet subset and TinyImageNet. Details are as follows: 

**Evaluation on ImageNet Subset** 

For the ImageNet experiment, we use ImageNet subset containing samples from 12 classes and a ResNet34 architecture. We train the model for 200 epochs with a learning rate of 0.01 with a decay rate of 0.1/75 epochs. We also employ 0.9 and 1e-4 for momentum and weight decay. In Table 1, we show the attack success rate/clean test accuracy(ASR/ACC) for 5 different backdoor attacks.


For removing the backdoor, we use 3% validation data and finetune the classification layer for 500 epochs. A learning rate of 0.001 has been employed with a decay rate of 0.95 per 10 epochs. For augmentations, we use ImageNetPolicy from AutoAugment [a]. The performance of NGF along with the other two methods: vanilla fine-tuning (FT) and ANP, is shown in Table 1. NGF consistently outperforms other methods in removing backdoor whereas keeping a satisfactory clean accuracy drop. For Badnets, we successfully purify the model (ASR of 0.18%) with a clean accuracy drop of 5.62%. However, it is observable that pruning-based techniques, e.g. ANP, may underperform in case of large models and datasets. On the other hand, vanilla FT performs reasonably well in removing backdoor. However, the large clean test accuracy drop is not desirable for a backdoor defense technique.  

**Table 1: Evaluation of NGF on ImageNet Subset**

|Defense Method|Clean Model|Badnets|Blend|Trojan |SIG|CLB|
|:----------|:----------|:----------|:----------|:----------|:----------|:----------|
|No Defense|0/85.16|100/82.74|98.57/83.11|99.15/82.34|96.73/81.97|94.72/80.85|
|ANP|0/**83.81**|23.27/74.18|65.91/76.58|40.06/75.10|38.14/**77.05**|11.23/74.92|
|FT|0/82.75|1.63/73.81|1.92/74.60|5.36/72.52|3.08/72.71|6.17/71.62|
|NGF|0/82.96|**0.18/77.12**|**1.69/77.25**|**3.82/76.16**|**2.18**/76.24|**5.81/75.17**|




Evaluation on TinyImageNet: 

We further created backdoor models trained on the TinyImageNet dataset. This dataset contains 100,000 images from 200 classes making it one of the diverse and challenging datasets. We use a poison rate of 5% for inserting backdoor into a ResNet34 architecture. We train the model for 150 epochs with a learning rate of 0.005 with a decay-rate of 0.1/60 epochs and a weight decay of 1e-4. For augmentation, we use Colorjitter(0.6, 0.65,0.3,0.1) and RandomHorizontalFlip. In Table 2, we show the attack success rate/clean test accuracy(ASR/ACC) for 5 different backdoor attacks.       

For purifying backdoor, we take 5% validation data and fine-tune the last layer for 500 epochs. As there are 200 classes, very few samples are available per class if we choose a validation size less than 5%. This seems to hurt clean test accuracy after purification. We use an initial learning rate of 0.01 with a decay rate of 0.65 per 50 epochs. For augmentation, we use Colorjitter(0.3, 0.35,0.2,0.07) and RandomHorizontalFlip. For ANP, we take the same number of validation samples and train for 2000 epochs with a learning rate of 0.02. For Vanilla FT, we fine-tune the whole network with the same training set up as NGF. Our proposed method achieves SOTA purification performance on TinyImageNet. 

**Table 2: Evaluation of NGF on TinyImageNet**

|Defense Method|Clean Model|Badnets|Blend|Trojan |SIG|CLB|
|:----------|:----------|:----------|:----------|:----------|:----------|:----------|
|No Defense|0/60.56|100/57.80|100/58.11|100/57.19|98.48/58.01|97.71/58.33|
|ANP|0/**57.29**|61.23/53.41|81.58/52.90|79.56/52.76|28.67/**53.71**|16.24/**53.18**|
|FT|0/56.20|3.84/51.58|1.76/49.22|6.77/50.62|5.02/50.18|5.61/49.68|
|NGF|0/56.64|**2.77/52.89**|**1.16/53.26**|**3.26/52.87**|**1.66**/52.54|**2.05**/52.80|

[a] Cubuk, Ekin D., et al. "Autoaugment: Learning augmentation policies from data." arXiv preprint arXiv:1805.09501 (2018).
 
***
***
**Response for Q3:**

In comparison to SGD, NGD takes additional time to compute the inverse of FIM $(F^{-1})$ [ref. Eqn 5] in each iteration. Although we fine-tune only one layer as compared to the full network for vanilla fine-tuning, the computational time does not decrease proportionally (to number of layers) due to the computational overhead of $(F^{-1})$. In our experiments, we use 500 epochs for both vanilla FT and NGF. However, we cannot use a pre-computed feature map (as the reviewer suggested) since we use *RandomHorizontalFlip* augmentation. In each iteration of training, the input changes as well as the feature map. However, we estimate the time required to calculate the feature map for 500 epochs, which is around 20 seconds.    

***

========================================================================

R2

Q1: The paper argues that the loss landscape of the purified model has a "similar curvature as the benign model". However, from Figure 1, it's a bit hard to draw such a conclusion. The three subfigures all have pretty similar smooth shapes, and the backdoored and purified ones even look more similar with the colors indicating the loss values at different perturbation magnitude combinations. How did you draw the conclusions in the paper? Since it’s not very clear visually, is there any quantitative evidence to support the claim of “the loss increment rate is steeper for backdoor model”?

Q2: The bold parts in Table 2 are a bit confusing. My understanding is that the best-performing one in each column is bolded, but there are some counterexamples. For example, the ACC with no defense is always the highest, but those are not bold. Even if we only consider the rows with defense, for the ACC column under SIG, FP gets a higher score but is also not bold. Similar issues are also observed in Table 3.

Q3: Is there an intuition of why only finetuning the last layer has very good performance? Is it because the task is simple, and even if the previous layers are troublesome, with the last layer trained by the benign validation set, it can achieve good performance? My main concern is that the earlier layers in the network are already contaminated by the backdoors, and it's impossible to remove such an effect by only finetuning the last layer. I would suggest another simple baseline to check against: instead of finetuning the last layer, re-initialize the last layer with random weights and train it with the validation set with a standard SGD optimizer. How is the performance?
========================================================================


***
**Response for Q1:**

To clarify the loss-landscape gradient, we have added a 1D loss-landscape for Badnets attack on CIFAR10 in the *Supplementary Material* section 5.1, Fig. 4. For generating this landscape we choose $\beta = 0$ [ref eq. 3] and only change the value of $\alpha$. From the figure, we observe that for a long range of $\alpha$ values (-0.5,0.5), both the benign and purified models have same type of flatness characteristics. As for the color code of Fig.1 in main paper, both the backdoored and purified model's landscapes are expected to be same color as the purified model's accuracy (ACC) is (almost) similar to the backdoored model's ACC. However, our goal is to flatten the surface as it helps reducing the attack success rate (ASR) significantly. Since NGF-based purified model achieves similar level of surface flatness as the benign model, ASR for benign and purified model becomes similar. We further verify this in 1D plot where backdoor and purified model is similar in terms of loss values, hence, similar ACC. On the other hand, benign and purified model has similar flatness characteristics, hence, similar ASR.

***
**Response for Q2:**

**Bold/Highlighting Criteria:** As we compare NGF with other defense methods, we disregard “No Defense” performances while highlighting the numeric figures. For a given attack, we highlight the lowest  numeric figure for ASR and highest numeric figure for ACC.  For example, we highlight  0.36% ASR for Blend attack which is the lowest in that column. We do the same thing for ACC.
We would like to thank the reviewer for pointing the “typo” out. In Table 2 of the main paper (on SIG column), we made a typo by making the ACC bold for NGF. Unfortunately, we did not notice the performance difference (between NGF and FP)  as the numeric figures are too close. It was an honest mistake from our part. However, we believe such mistakes does not take place in Table 3.  

***
**Response for Q3:**

*Intuition:* In general, the DNN backbone generates the feature map for an input instance, and the classification layer classifies the map to a specific class. Let us consider the map generation for: (i) clean samples, and (ii) poisonous samples. Since the backdoor model always performs like a benign model for clean input, keeping the DNN backbone unchanged for case (i) absolutely makes sense. Now consider case (ii), an adversary may contaminate weights to generate the desire feature map in favor of the target class. We conjecture that the classifier plays a big role in prioritizing the features corresponding to a poisonous input in a way such that the model predicts the target class. Therefore, effective fine-tuning (with the help of NGD) of the classification layer can remove the backdoor. Throughout our empirical evaluation, we observe similar phenomena.

*Experiment with re-initialize the last layer with random weights:* Following the reviewer’s suggestion, we performed the following experiments revealing that SGD completely fail to remove the backdoor (experimental results reported in the following table). However, NGF successfully removes the backdoor in this case too. Intuitively, SGD optimizes the model with random initialized last layer weights to a *bad local minima* which favors the poisoned samples to predict the target label. In contrast, NGD optimizes to global minima canceling the prior effect of backdoor in the model.  

For experimental evaluation, we take 5 different backdoored models trained on CIFAR10.

**Table 3: Performance  evaluation of NGF and SGD while re-initializing  the last layer with random weights**
||Badnet|Trojan|Blend|CLB|SIG|
|:----------------|:----------------|:----------------|:---------------|:----------------|----------------:|
|No Defense|100/90.93|100/90.67|100/93.98|98.72/89.18|99.75/88.64|
|SGD|93.51/89.35|99.63/87.55|100/92.21|98.01/84.01|98.83/87.12|
|NGF|3.34/89.65|18.78/84.21|0.33/86.39|4.45/82.5|1.25/77.95|

***


========================================================================

R3

========================================================================

Can you provide experimental results for ImageNet?


What's your accuracy drop if the backdoors are inserted without any accuracy drop?
Does he mean the backdoor model has same clean ACC as the clean model? We will have accuracy drop to achieve the desired attack success rate. However, we can try for Badnets, Blend and Trojan. 

 How do you measure removal? Is it sufficient for backdoored images to be classified as a non-target class or does it have to be the original class?

------------------------------------------------------------------------------------------


**Response for first question:**
We have evaluated our method on ImageNet subset and TinyImageNet. 

**ImageNet Subset** 
For the ImageNet experiment, we use ImageNet subset containing samples from 12 classes and a ResNet34 architecture. We train the model for 200 epochs with a learning rate of 0.01 with a decay rate of 0.1/75 epochs. We also employ 0.9 and 1e-4 for momentum and weight decay. In Table 1, we show the attack success rate/clean test accuracy(ASR/ACC) for 5 different backdoor attacks.

For removing the backdoor, we use 3% validation data and finetune classification layer for 500 epochs. A learning rate of 0.001 has been employed with a decay rate of 0.95 per 10 epochs. For augmentations, we use ImageNetPolicy. The performance of NGF along with vanilla fine-tuning (FT) and ANP, is shown in Table 1. NGF consistently outperforms other methods in removing backdoor whereas keeping a satisfactory clean accuracy drop. For Badnets, we successfully purify the model (ASR of 0.18%) with a clean accuracy drop of 5.62%. However, it is observable that pruning-based techniques, e.g. ANP, may underperform in case of large models and datasets. On the other hand, vanilla FT performs reasonably well in removing backdoor. However, the large clean test accuracy drop is not desirable for a backdoor defense technique.  

**Table 1: Evaluation on ImageNet Subset**
||Clean Model|Badnets|Blend|Trojan |SIG|CLB|
|:---|:---|:---|:---|:---|:---|---:|
|No Defense|0/85.16|100/82.74|98.57/83.11|99.15/82.34|96.73/81.97|94.72/80.85|
|ANP|0/**83.81**|23.27/74.18|65.91/76.58|40.06/75.10|38.14/**77.05**|11.23/74.92|
|FT|0/82.75|1.63/73.81|1.92/74.60|5.36/72.52|3.08/72.71|6.17/71.62|
|NGF|0/82.96|**0.18/77.12**|**1.69/77.25**|**3.82/76.16**|**2.18**/76.24|**5.81/75.17**|

**TinyImageNet:** 
We further created backdoor models trained on the TinyImageNet dataset. This dataset contains 100,000 images from 200 classes making it one of the diverse and challenging datasets. We use a poison rate of 5% for inserting backdoor into a ResNet34 architecture. We train the model for 150 epochs with a learning rate of 0.005 with a decay-rate of 0.1/60 epochs and a weight decay of 1e-4. For augmentation, we use Colorjitter and RandomHorizontalFlip. In Table 2, we show ASR/ACC for 5 different attacks.       

For purifying backdoor, we take 5% validation data, fine-tune the last layer for 500 epochs. As there are 200 classes, very few samples are available per class if we choose a validation size less than 5%. This seems to hurt clean test accuracy after purification. We use an initial learning rate of 0.01 with a decay rate of 0.65/50 epochs. For augmentation, we use Colorjitter and RandomHorizontalFlip. For ANP, we take the same number of validation samples and train for 2000 epochs with a learning rate of 0.02. For Vanilla FT, we fine-tune the whole network with the same training set up as NGF. NGF achieves SOTA purification performance on TinyImageNet. 

**Table 2: Evaluation on TinyImageNet**
||Clean Model|Badnets|Blend|Trojan |SIG|CLB|
|:---|:---|:---|:---|:---|:---|---:|
|No Defense|0/60.56|100/57.80|100/58.11|100/57.19|98.48/58.01|97.71/58.33|
|ANP|0/**57.29**|61.23/53.41|81.58/52.90|79.56/52.76|28.67/**53.71**|16.24/**53.18**|
|FT|0/56.20|3.84/51.58|1.76/49.22|6.77/50.62|5.02/50.18|5.61/49.68|
|NGF|0/56.64|**2.77/52.89**|**1.16/53.26**|**3.26/52.87**|**1.66**/52.54|**2.05**/52.80|

***

**Response for second question:**

Creating a backdoor model with the same accuracy (ACC) as the benign model is a very challenging task. This is due to the fact that same number of clean samples are not available for both scenarios. Furthermore, the model has to learn features from both the clean and poisonous samples. Therefore, compared to a benign model, a backdoor model has to learn two tasks. Even though deep neural network is very powerful at learning representations, an additional task (backdoor insertion) for the backdoor model limits its generalization performance (ACC) on the clean samples. 

For some attacks, e.g. FC, Trojan, etc., the ACC becomes lower than usual while performing a strong and successful attack. We, however, aim to create a backdoor model with low ACC drop by setting the poison rate to 1%. The closest backdoor model we get is for the Blend attack on CIFAR10 dataset (95.04% vs 95.26%). We report the accuracy drop in Table 4.

**Table 4: Clean Test Accuracy (%) drop of NGF if backdoors are inserted with low accuracy drop**
|Defense Method|Benign Model|Badnets|Blend |Trojan |
|:----------|:----------|:----------|:----------|:----------|----------:|
|No Defense|0/95.26|100/93.8|100/95.04|100/91.11|
|NGF|0/92.27|1.08/89.23|0.51/92.61|1.96/86.12|
|Drop|0/2.99|98.92/4.57|99.49/2.43|98.04/4.99|
***

**Response for third question:**

In standard removal measurement, it is sufficient for backdoored images to be classified as a non-target class. As we calculate ASR after removal, our evaluation follows standard measurement. However, we also consider the reviewer's second point. We define the correction rate (CR) as the percentage of poisonous samples correctly classified to their original classes. We define the method with the highest value of CR as the best performing or SOTA method. We use CIFAR10 dataset and 4 different attacks for demonstration. It can be observed from Table 5 that our method obtains SOTA correction performance for most of these attacks.

**Table 5: Correction rate(%) for different defense techniques.**
|Defense Method|Badnet|Trojan|CLB|SIG|
|:---------------|:---------------|:---------------|:---------------|---------------:|
|No Defense|0|0|0|0|
|Vanilla FT|85.74|80.52|84.72|43.35|
|ANP|85.56|80.69|82.04|**45.64**|
|NGF (Ours)|**86.42**|**80.85**|**85.63**|45.18|




=========================

**Response for Q1:**
NGD is a loss surface geometry-aware optimizer that helps it to skip local minima. In case of one layer fine-tuning, the optimization problem intuitively becomes an under-parameterized model containing **bad local minima**. In such a case, SGD and its variants most probable get stuck in those bad local minima performing poorly for the optimization problem [18,19]. In contrast, due to the geometry awareness of NGD, it can easily avoid local minima. Therefore, NGD performs so well than the first-order optimizers. 

From another point of view, NGD helps to generate a flat weight landscape surface which makes the fine-tuned DNN model more robust against the poisoned samples. We hypothesize that the loss surface geometry awareness of NGD helps it to flatten the landscape. The experimental loss landscapes corresponding to our hypothesis are presented in Fig. 1 which support our claim.
***
**Response for Q2:** We have evaluated our method on ImageNet subset and TinyImageNet. 

**ImageNet Subset** 
For the ImageNet experiment, we use ImageNet subset containing samples from 12 classes and a ResNet34 architecture. We train the model for 200 epochs with a learning rate of 0.01 with a decay rate of 0.1/75 epochs. We also employ 0.9 and 1e-4 for momentum and weight decay. In Table 1, we show the attack success rate/clean test accuracy(ASR/ACC) for 5 different backdoor attacks.

For removing the backdoor, we use 3% validation data and finetune classification layer for 500 epochs. A learning rate of 0.001 has been employed with a decay rate of 0.95 per 10 epochs. For augmentations, we use ImageNetPolicy. The performance of NGF along with vanilla fine-tuning (FT) and ANP, is shown in Table 1. NGF consistently outperforms other methods in removing backdoor whereas keeping a satisfactory clean accuracy drop. For Badnets, we successfully purify the model (ASR of 0.18%) with a clean accuracy drop of 5.62%. However, it is observable that pruning-based techniques, e.g. ANP, may underperform in case of large models and datasets. On the other hand, vanilla FT performs reasonably well in removing backdoor. However, the large clean test accuracy drop is not desirable for a backdoor defense technique.  

**Table 1: Evaluation on ImageNet Subset**
||Clean Model|Badnets|Blend|Trojan |SIG|CLB|
|:---|:---|:---|:---|:---|:---|---:|
|No Defense|0/85.16|100/82.74|98.57/83.11|99.15/82.34|96.73/81.97|94.72/80.85|
|ANP|0/**83.81**|23.27/74.18|65.91/76.58|40.06/75.10|38.14/**77.05**|11.23/74.92|
|FT|0/82.75|1.63/73.81|1.92/74.60|5.36/72.52|3.08/72.71|6.17/71.62|
|NGF|0/82.96|**0.18/77.12**|**1.69/77.25**|**3.82/76.16**|**2.18**/76.24|**5.81/75.17**|

**TinyImageNet:** 
We further created backdoor models trained on the TinyImageNet dataset. This dataset contains 100,000 images from 200 classes making it one of the diverse and challenging datasets. We use a poison rate of 5% for inserting backdoor into a ResNet34 architecture. We train the model for 150 epochs with a learning rate of 0.005 with a decay-rate of 0.1/60 epochs and a weight decay of 1e-4. For augmentation, we use Colorjitter and RandomHorizontalFlip. In Table 2, we show ASR/ACC for 5 different attacks.       

For purifying backdoor, we take 5% validation data, fine-tune the last layer for 500 epochs. As there are 200 classes, very few samples are available per class if we choose a validation size less than 5%. This seems to hurt clean test accuracy after purification. We use an initial learning rate of 0.01 with a decay rate of 0.65/50 epochs. For augmentation, we use Colorjitter and RandomHorizontalFlip. For ANP, we take the same number of validation samples and train for 2000 epochs with a learning rate of 0.02. For Vanilla FT, we fine-tune the whole network with the same training set up as NGF. NGF achieves SOTA purification performance on TinyImageNet. 

**Table 2: Evaluation on TinyImageNet**
||Clean Model|Badnets|Blend|Trojan |SIG|CLB|
|:---|:---|:---|:---|:---|:---|---:|
|No Defense|0/60.56|100/57.80|100/58.11|100/57.19|98.48/58.01|97.71/58.33|
|ANP|0/**57.29**|61.23/53.41|81.58/52.90|79.56/52.76|28.67/**53.71**|16.24/**53.18**|
|FT|0/56.20|3.84/51.58|1.76/49.22|6.77/50.62|5.02/50.18|5.61/49.68|
|NGF|0/56.64|**2.77/52.89**|**1.16/53.26**|**3.26/52.87**|**1.66**/52.54|**2.05**/52.80|
***
**Response for Q3:**
In comparison to SGD, NGD takes additional time to compute the inverse of FIM $(F^{-1})$ [ref. Eqn 5] in each iteration. Although we fine-tune only one layer as compared to the full network for vanilla fine-tuning, the computational time does not decrease proportionally (to number of layers) due to computational overhead of $(F^{-1})$. In our experiments, we use 500 epochs for both vanilla FT and NGF. However, we cannot use a pre-computed feature map (as the reviewer suggested) since we use *RandomHorizontalFlip* augmentation. In each iteration of training, the input changes as well as the feature map. As a result, we could not perform such experiment.

==> related_work_aug.tex <==
\section{Related Work}
\textit{Backdoor Attack:} A substantial number of studies have investigated the possibility of backdoor attacks after the initial studies~\cite{gu2017badnets,chen2017targeted,liu2017neural} probed their existence. The nature of these attacks vary based on the rendered trigger type, injected malicious behavior, the stealthiness of the backdoor infusion approach and the attacker insights about the model~\cite{guo2021aeva}. Generally, backdoor attacks are categorized in two types: clean-label attacks, and poison-label attacks. Clean-label backdoor attack doesn't alter the label, while poison-label attack aim at specific target classes such that DNN misclassifies to those classes in presence of trigger~\cite{li2021neural}. As for the trigger types, researchers have studied numerous types of triggering patterns in their respective attacks~\cite{gu2019badnets,chen2017targeted, turner2018clean, zhong2020backdoor, li2020backdoor, liu2020reflection}. Such triggers can exist in a form of dynamic patterns~\cite{li2020backdoor} or as simple as a single pixel~\cite{tran2018spectral}. Some of the more complex backdoor triggers that have been proposed in the literature are sinusoidal strips~\cite{barni2019new}, human imperceptible noise~\cite{zhong2020backdoor},natural reflection~\cite{liu2020reflection}, adversarial patterns~\cite{zhao2020clean}, and blending backgrounds~\cite{chen2017targeted}.

\textit{Backdoor Defense:}  Generally, the backdoor defense mechanism can be categorized into types: methods mitigating the backdoor attack during the test time, and methods abating the backdoor affect with the training~\cite{guo2021aeva,li2021neural}.
In the first approach, the defender doesn't have an access to the training. To diagnose and perform poison cleansing, the trigger can be estimated via adversarial perturbation~\cite{wang2019neural} or generative adversarial network(GAN)~\cite{qiao2019defending}. After constructing the trigger, pruning can be performed on the neurons sensitive to these triggers. However, trigger re-synthesis has become extremely challenging with the attacks generated via complex triggering patterns~\cite{wu2021adversarial}. With respect to outlying the poisoned data points, detection and filtration is performed either in the feature space~\cite{gao2019strip, koh2017understanding, ma2019nic, tran2018spectral} or in the input space~\cite{diakonikolas2019sever,gao2019strip,steinhardt2017certified}. Regarding training techniques to mitigate the backdoor attack,   
the researchers have proposed numerous defense methods through input pre-processing~\cite{liu2017neural}, poison-suppression ~\cite{hong2020effectiveness}, model diagnosis~\cite{li2020backdoor}, network pruning~\cite{wu2020adversarial,liu2017neural}, and model reconstruction ~\cite{zhao2020bridging}.  



